Reimplementing the Wheel: Teaching Compilers with a Small Self-Contained One

We report on a one-semester compiler construction course based on the idea of implementing a small self-contained compiler for a small model language from scratch, not using other compiler construction frameworks. The course is built around an evolving family of languages with increasing expressiveness and complexity, which finally is crowned by a language with first-class functions, S-expressions, pattern matching, and garbage collection. The code generation technique is based on the idea of symbolic interpreters, which allows to implement a robust albeit not a very efficient native code generator. We give the motivation for the course, describe its structure, and report some results of teaching based on students' post-course surveys.

==> eptcsdata.tex <==
\providecommand{\firstpage}{22}
\providecommand{\publicationstatus}{P. Achten \& E. Machkasova  (Eds.): Trends in\\
Functional Programming in Education (TFPIE) 2021/22
\\
EPTCS 363, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.363.2}{10.4204/EPTCS.363.2}}
\pdfoutput=1

